Story Disambiguation: Tracking Evolving News Stories across News and Social Streams

Following a particular news story online is an important but difficult task, as the relevant information is often scattered across different domains/sources (e.g., news articles, blogs, comments, tweets), presented in various formats and language styles, and may overlap with thousands of other stories. In this work we join the areas of topic tracking and entity disambiguation, and propose a framework named Story Disambiguation - a cross-domain story tracking approach that builds on real-time entity disambiguation and a learning-to-rank framework to represent and update the rich semantic structure of news stories. Given a target news story, specified by a seed set of documents, the goal is to effectively select new story-relevant documents from an incoming document stream. We represent stories as entity graphs and we model the story tracking problem as a learning-to-rank task. This enables us to track content with high accuracy, from multiple domains, in real-time. We study a range of text, entity and graph based features to understand which type of features are most effective for representing stories. We further propose new semi-supervised learning techniques to automatically update the story representation over time. Our empirical study shows that we outperform the accuracy of state-of-the-art methods for tracking mixed-domain document streams, while requiring fewer labeled data to seed the tracked stories. This is particularly the case for local news stories that are easily over shadowed by other trending stories, and for complex news stories with ambiguous content in noisy stream environments.

==> 4-eval-old.tex <==
%!TEX root = main.tex

In this section, we discuss our methodology for gathering labeled data, and show extensive experiments analyzing the building blocks of our techniques. We also compare our Story Disambiguation framework to the state-of-the-art (SOTA) story tracking approaches.

\subsection{Labeled Data Collection}\label{sec:label-data}
There are several labeled datasets specifically created for training and evaluating Topic Detection and Tracking (TDT) methods, such as TDT1\footnote{\url{https://catalog.ldc.upenn.edu/LDC98T25}}, TDT4\footnote{\url{https://catalog.ldc.upenn.edu/LDC2005T16}}, and TDT5\footnote{\url{https://catalog.ldc.upenn.edu/LDC2006T19}}. 
They consist of either news articles or the transcripts of the news broadcast, and their content is long and formal. 
In our problem setting, we would like to track diverse types of data for news stories, including formal articles and blogs, as well as noisy tweets and comments. 
Unfortunately, we did not find a dataset that contains both formal articles and social posts regarding the same set of news stories.
The existing datasets contain either one or the other data type, and combining multiple datasets is not feasible because they are not labeled with the same set of news stories.
Therefore, we create a labeled dataset using human annotators.
We first collect data from the news domain from multiple sources for over one year, and then we select 9 news stories for labeling.
We make the dataset that contains labeled news articles and tweets for each of the 9 stories available to the research community\footnote{\url{https://gitlab.com/claireshi/story-disambiguation-data.git}}.

\textbf{Data Collection Sources.}
Limited by the accessibility and the labeling difficulty, we collect two distinct types of data for news stories: news articles and tweets. 
We monitor the RSS feeds of some major news publishers, including BBC, Reuters, The Irish Times, etc., for one year, and collect around 180K news articles on a variety of topics.
For the tweets, we collect data using the Twitter Streaming API with dynamically updated keyphrases that are extracted from recent news articles and reflect the current news topics.
In average, we collect around 1 million tweets per day for over a year.
For more details on this process, please see \cite{shi:www16}.
%The methodology for collecting news articles and tweets is similar to that used in Hashtagger+ in Chapter \ref{chap:hashtagger}.
%, and the method for extracting dynamic keyphrases is detailed in Section \ref{sec:keyphrases}.


\textbf{Selecting News Stories for Labeling.}
To properly test the Story Disambiguation framework on many types of news stories, we selected a diversity of stories with 4 different combinations of characteristics for labeling.
The attributes of news stories include:
\begin{enumerate}
    \item The life span of the story, varied between few days to few years.
    \item The popularity of the story, reflected by the number of articles and tweets related to it.
    \item The locality of the story: whether it attracts attention locally or globally. This is decided manually by analyzing the coverage and reach of a story. Global stories are usually popular as well.
    \item The complexity of the story, regarding the number of entities related to the story. Big news stories involve many people, companies, organizations, etc., while other stories are only reported with limited details and include fewer entities.
\end{enumerate}

\begin{table*}[t]
\centering
\caption{The characteristics of the 9 collected and labeled news stories.}
\label{table:9-stories}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|}\hline
News Story                  & Duration (weeks) & Popularity & Locality & Complexity \\\hline\hline
Cyclone Debbie              & 1                & Low        & Global   & Low        \\\hline
Kim-Jong-Nam Death          & 8                & Low        & Local    & Low        \\\hline
Orly Airport Attack         & 1                & Low        & Local    & Low        \\\hline
South Africa President Zuma & 52               & Low        & Local    & High     \\\hline
EU Migrant Crisis           & 52               & High       & Global   & High     \\\hline
Irish Water Charges         & 52               & High       & Local    & High     \\\hline
Trump Healthcare            & 21               & Low        & Global   & High       \\\hline
London Attack               & 1                & High       & Global   & High       \\\hline
Irish General Election 2016 & 4                & High       & Local    & High       \\\hline
\end{tabular}%}
\end{table*}


Table \ref{table:9-stories} shows 9 selected stories with their characteristics, ordered by the complexity of the stories. 
Among the 9 stories, 3 of them only lasted for at most a week, while 3 others lasted for a year or more. 
Some stories are viral, with hundreds of articles and tens of thousands of tweets, labeled in a manner we explain in the next section. 
Half of the stories attract attention worldwide, while the other half are only of interest locally. 
Regarding the story complexity, we collected stories in two complexity level: low, and high.
A low complexity story only has 1 or 2 important entities (e.g., peoples' names or short phrases that appear in many of the articles and tweets of that story), while high complexity stories have more than 20. The total number of entities, regardless of their frequency in the story, is more than a few hundred for a  complex story. 

\textbf{Data Collection and Labeling.} We collect relevant news articles and tweets for the 9 selected news stories.
For each story, we manually select few keyphrases/words from the story and use them in an article pre-filtering step. 
We retrieve articles with the matching keywords in their headline or sub headline from our collection, and let a human annotator label this subset of articles manually.
The keywords filtering step significantly reduces the amount of labeling work on the annotator, reducing from the entire 180K collection down to few hundred articles per story, but with the compromise of not retrieving all relevant articles.
Regarding labeling tweets, we only label tweets as relevant to the target story if they contain the story specific hashtags (e.g., \#ge16 for Irish General Election 2016).
We identified 1 - 3 story specific hashtags, and use them as the label of the tweets.
Obviously, a lot of relevant tweets that do not contain the hashtag are missing from our positive labeled set, but it is not feasible for annotators to label tens of thousands of tweets for each story.
Table \ref{table:9-stories-keyphrases-hashtags} shows the keyphrases and the hashtags we choose for the 9 selected stories and the number of relevant articles and tweets retrieved per story.

\begin{table*}[]
\centering
\caption{The manually selected keyphrases and hashtags used to collect articles and tweets for the 9 selected stories.}
\label{table:9-stories-keyphrases-hashtags}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{3.5cm}|p{4cm}|p{2.7cm}|c|c|}\hline
News Story                  & Keywords/Keyphrases & Hashtags & Articles & Tweets \\\hline\hline
Cyclone Debbie              & cyclone debbie, flood, australia               & \#cyclonedebbie  & 21 & 1979   \\\hline
Kim-Jong-Nam Death          & kim jong-nam, north korea, malaysia                & \#kimjongnam    & 71 & 3518    \\\hline
Orly Airport Attack         & orly, airport, paris         & \#orly & 18 & 2605 \\\hline
South Africa President Zuma & south africa, zuma, cabinet               & \#cabinetreshufle, \#zuma     & 74 & 1005   \\\hline
EU Migrant Crisis           & migrant crisis, europe, eu               & \#migrantcrisis   & 809 & 5000  \\\hline
Irish Water Charges         & irish water, water charges              & \#watercharges, \#right2water, \#irishwater   & 389 & 5000  \\\hline
Trump Healthcare            & trump, healthcare, health              & \#trumpcare   & 42 & 3677   \\\hline
London Attack               & westminster attack, london attack               & \#prayforlondon, \#westminster, \#londonattack   & 140 & 2244    \\\hline
Irish General Election 2016 & general election, ireland, irish                & \#ge16    & 908 & 40K  \\\hline
\end{tabular}%}
\end{table*}

After gathering a collection of relevant articles and tweets per story as positive examples, we randomly select an equal number of irrelevant articles and tweets that are published in the same time window as the story, and label them as negative examples.
Thus, we get 9 sets of labeled data, one set for each story, with only two types of labels in each set: relevant or irrelevant to that particular story.

In the following experiments, we use the Irish General Election 2016 (GE16) story as a labeled set for training and validation, and use the 8 remaining labeled story datasets as the test data.
We show the detailed experiment setup in the following sections.

\subsection{Training the Learning-to-Rank Model}\label{sec:training}

%In this section, we show the training the Story Disambiguation model on the GE16 dataset.

As discussed in Section \ref{sec:classifier-feature}, to construct story-doc pairs for training our L2R model, we prepare the story representation $S$ and the incoming text $m$ from stream $T$ separately, then pair them together.
We first create three story representations by randomly sampling 3 small groups of relevant articles + tweets for the \emph{story docs}, and construct the entity graph $G$ following the steps presented in Section \ref{sec:entity-graph}.
These three groups consist of a different number of relevant data, as shown in Table \ref{table:construct-graph}, simulating different stories.
The total number of nodes and edges in the constructed graphs vary accordingly.

\begin{table*}[t]
\centering
\caption{Three settings for constructing \emph{story docs} and entity graphs $G$ for training}
\label{table:construct-graph}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|}
\hline
        & Articles in \emph{story docs} & Tweets in \emph{story docs} & Nodes in $G$ & Edges in $G$ \\ \hline
GE16 story 1 & 5        & 20     & 48      &  74     \\ \hline
GE16 story 2 & 50       & 200    &  378   &  1259   \\ \hline
GE16 story 3 & 100      & 400    & 657    &  2742  \\ \hline
\end{tabular}%}
\end{table*}

We then create the document set by selecting all relevant articles ($0.9$K) plus a random sample of relevant tweets ($1.8$K) of the story as the positive data ($2.7$K in total), and randomly selecting the same number of irrelevant articles and tweets as the negative data.
Thus, we have a labeled document set of size $5.4$K, with an equal number of true and false (relevant/irrelevant) examples.
Finally, we pair the three story representations to each of the documents. 
Thus, we have $16.2$K ($3\times 5.4$) training data representing the story-doc relationship, mixing different sizes of stories and different types of documents.


%\subsection{Binary Classifier Selection}\label{sec:compare-classifiers}
%
%\begin{table*}[]
%\centering
%\caption{Comparing 8 different pointwise learning-to-rank classifiers in term of Precision, Recall and F1.}
%\label{table:story-classifiers}
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%Classifier              & Precision & Recall & F1    & Runtime(s) \\ \hline
%Random Forest           & \textbf{0.873}     & \textbf{0.850}  & \textbf{0.863} & 2.46      \\ \hline
%Logistic Regression     & 0.797     & 0.745  & 0.776 & 0.47       \\ \hline
%K-Neighbors             & 0.845     & 0.832  & 0.840 & 1.30      \\ \hline
%Multilayer Perceptron   & 0.864     & 0.773  & 0.828 & 82.95      \\ \hline
%LinearSVC               & 0.797     & 0.739  & 0.774 & 1.62       \\ \hline
%Gradient Boosting       & 0.876     & 0.842  & 0.862 & 14.22      \\ \hline
%AdaBoost                & 0.854     & 0.823  & 0.840 & 7.07       \\ \hline
%Multinomial Naive Bayes & 0.810     & 0.754  & 0.774 & 0.09       \\ \hline
%\end{tabular}
%\end{table*}
%
%In this section, we investigate different L2R algorithms to study which are the most appropriate for the story tracking setting.
%The pointwise L2R methods are the most suitable for binary classes scenario in dynamic problem settings \cite{Agarwal2012,shi2017hashtagger}, hence, in this section, we only study the pointwise approaches.
%
%\textbf{Experiment Setup.} We use the scikit-learn (sklearn)\footnote{\url{http://scikit-learn.org/stable/index.html}} library for 8 pointwise classifiers. 
%We use the 16.2K labeled data extracted from the GE16 dataset, and test the 8 pointwise classifiers using 10-fold cross-validation.
%The classifiers use all 13 features presented in Section \ref{sec:feature-engineering}.
%We measure the performance of each classifier in standard Information Retrieval measurements: Precision, Recall, F1.
%We are also interested in the total runtime of the classifiers.
%
%\textbf{Result.} The classification performance is shown in Table \ref{table:story-classifiers}.
%Among the 8 classifiers, we find the RandomForest to be the best one in terms of Precision, Recall, and F1.
%The second most accurate classifier is Gradient Boosting. However, it is too slow comparing to RandomForest (14.22s vs. 2.46s).
%K-Neighbors is another promising classifier with good accuracy and fast runtime.
%All other classifiers are either not as accurate or too slow in comparison to RandomForest.

\subsection{Feature Evaluation}\label{sec:feature-evaluation}

\begin{table*}[]
\centering
\caption{Evaluating the classification performance of different combinations of relevance features. The features are described in Table \ref{table:features}}
\label{table:story-features}
\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Features} & Precision & Recall & F1 & Runtime(s)    \\ \hline
Story/Doc Alone (1-4)         & 0.590     & 0.628  & 0.592  & 1.29\\ \hline
Story/Doc+Tf-idf (1-4,9)      & 0.776     & 0.743  & 0.765 & 1.90\\ \hline
Text-Based (1-9)               & 0.838     & 0.807  & 0.825 & 1.93\\ \hline
Graph-Based (1-4,9-13)         & \textbf{0.881}     & \textbf{0.848}  & \textbf{0.867} & 2.34\\ \hline
All Features(1-13)        & 0.875     & 0.847  & 0.863 & 2.45\\ \hline

\end{tabular}
\end{table*}


\begin{figure*}[]
	\centering 
    \includegraphics[width=0.9\linewidth]{story_figs/feature_box_plot.eps}
%    \vspace{-0.4cm}
    \caption{The box plots of true and false labels of the 13 features used in the L2R model. Features entity\_overlap, cosine\_simi, entity\_simi and entity\_simi\_avg seem to be most useful for discriminating between relevant and irrelevant pairs, showing the impact of the entity-based, text-based, and graph-based features.}
    \label{fig:story-features}

\end{figure*}

In this section, we present a thorough analysis of the influence of different features on learning a story-doc relevance classifier.
Figure \ref{fig:story-features} shows the distribution in the 16.2K labeled data of the 13 features presented in Section \ref{sec:feature-engineering}.
The first 4 features only describe the story or the target document alone. Hence, we see similar distributions between the True and False labels.
The remaining features describe the association strength of a story and a document.
The entity\_overlap features correspond to features 5-8 in Table \ref{table:features}, while entity\_simi features to features 10-13.

\textbf{Experiment Setup.} We use the same experimental setup as in the previous section.
A RandomForest classifier is trained on 16.2K labeled data, with a different combination of the 13 features.
The evaluation is done via 10-fold cross-validation.
Again, we use Precision, Recall, and F1 to evaluate classification quality, and record runtime for using different features (feature extraction time is not included).

\textbf{Result.}
We test 5 combinations of the 13 features.
Experiment results are shown in Table \ref{table:story-features}.
Story/Document Alone refers to the 4 features that only describe the story or the target document.
Since they do not capture the relevance between the story-doc pairs, using only such features gives poor classification results.
With an extra tf-idf feature, which is used in most text mining techniques, we increase the F1 to 0.765.
Text-Based features include the 4 entity\_overlap features presented in Table \ref{table:features}.
They are extracted from the disambiguated text content, and significantly improve the classification quality by increasing the F1 to 0.825.
On the other hand, the Graph-Based features include the 4 entity\_simi features that are extracted using the node weights of story graph $G$.
By comparing the Text-Based features to the Graph-Based, we demonstrate the importance of employing the story-entity graph representation to describe the story.
The classification quality increases considerably (F1 0.867 vs. 0.825).
We also notice that when using all 13 features, the Precision, Recall and F1 slightly decrease comparing to the Graph-Based, showing that the Graph-Based features can replace the Text-Based features.
To ensure the robustness of the model in different datasets, we use all 13 features.

\subsection{Evaluating the Semi-Supervised Selection Methods}\label{sec:ssl-compare}
%\afterpage{
%\begin{longtable}[t]{|p{2cm}|c|c|c|c|c|c|c|c|c|}
%\caption{Comparing the 5 semi-supervised selection (SSS) techniques using 8 test story datasets. The N and E refer to number of nodes and edges of the initial story graph $G_{t_0}$. The N$\prime$ and E$\prime$ refer to the number of nodes and edges of the updated story graph when reaching the end of stream $T$.} \label{table:sss-compare} \\
%\hline
%Story                                        & N & E             & SSS    & N$\prime$ & E$\prime$ & Precision & Recall & F1   & Time \\ \hline
%\endfirsthead
%
%\multirow{5}{2cm}{Cyclone Debbie}              & \multirow{5}{*}{9}  & \multirow{5}{*}{12}   & None & 9               & 12             & 0.91       & \textbf{1}     & 0.95    &    21  \\ \cline{4-10} 
%                                             &                    &                     & Acc    & 99             & 313            & 0.93      & 0.98   & 0.96 &  8   \\ \cline{4-10} 
%                                             &                    &                     & Rev    & 125            & 345            & 0.96       & 0.98   & 0.97 & 248  \\ \cline{4-10} 
%                                             &                    &                     & RR     & 130            & 400            & \textbf{0.97}      & 0.98   & \textbf{0.98} &   234   \\ \cline{4-10} 
%                                             &                    &                     & AR     & 97             & 307            & 0.95      & 0.98   & 0.96 &   30   \\ \hline\hline
%\multirow{5}{2cm}{Kim Jong-Nam Death}          & \multirow{5}{*}{6}  & \multirow{5}{*}{9}   & None &               6 &    9            &  0.91         &   0.97     &     0.94 &   21   \\ \cline{4-10} 
%                                             &                    &                     & Acc    & 96            & 433            & \textbf{0.97}      & 0.99    & \textbf{0.98}  &  21    \\ \cline{4-10} 
%                                             &                    &                     & Rev    & 115            & 514            & \textbf{0.97}       & \textbf{1}    & \textbf{0.98}  &  777    \\ \cline{4-10} 
%                                             &                    &                     & RR     & 98            & 393            & \textbf{0.97}       & \textbf{1}    & \textbf{0.98}  & 816     \\ \cline{4-10} 
%                                             &                    &                     & AR     & 87             & 403            & \textbf{0.97}       & \textbf{1}    & \textbf{0.98}  &  102    \\ \hline\hline
%\multirow{5}{2cm}{Orly Airport Attack}         & \multirow{5}{*}{4}  & \multirow{5}{*}{6}   & None &               4 &   6             &   0.92        &  0.95      &     0.93 &  12    \\ \cline{4-10} 
%                                             &                    &                     & Acc    & 59             & 129             & 0.95     & \textbf{0.95}   & \textbf{0.95} &   10   \\ \cline{4-10} 
%                                             &                    &                     & Rev    & 62             & 132            & \textbf{0.96}      & 0.91   & 0.93 &   404   \\ \cline{4-10} 
%                                             &                    &                     & RR     & 67             & 165            & \textbf{0.96}      & 0.93   & \textbf{0.95} &   422   \\ \cline{4-10} 
%                                             &                    &                     & AR     & 45             & 100             & 0.94      & 0.93   & 0.93 &   45   \\ \hline\hline
%\multirow{5}{2cm}{South Africa President Zuma} & \multirow{5}{*}{8}  & \multirow{5}{*}{19}   & None &               8 & 19               &  0.80         &  0.84      &     0.80 &  5    \\ \cline{4-10} 
%                                             &                    &                     & Acc    & 184            & 597            & 0.95      & 0.70   & 0.80 &  8    \\ \cline{4-10} 
%                                             &                    &                     & Rev    & 167            & 642            & 0.95      & 0.57   & 0.72 &  89    \\ \cline{4-10} 
%                                             &                    &                     & RR     & 126            & 440            & \textbf{0.96}      & 0.71   & 0.81 &   92   \\ \cline{4-10} 
%                                             &                    &                     & AR     & 121            & 485            & \textbf{0.96}      & \textbf{0.71}   & \textbf{0.82} &   18   \\ \hline\hline
%\multirow{5}{2cm}{EU Migrant Crisis}           & \multirow{5}{*}{2}  & \multirow{5}{*}{1}   & None &               2 &    1            &  \textbf{0.92}         &  0.47      &     0.62 & 61     \\ \cline{4-10} 
%                                             &                    &                     & Acc    & 530            & 2091           & 0.91      & 0.57   & 0.70 &    68  \\ \cline{4-10} 
%                                             &                    &                     & Rev    & 1024           & 4714           & 0.91      & \textbf{0.67}   & 0.77 &  2798    \\ \cline{4-10} 
%                                             &                    &                     & RR     & 168            & 406            & 0.89      & 0.66   & 0.76 &  1534    \\ \cline{4-10} 
%                                             &                    &                     & AR     & 873            & 4219           & \textbf{0.92}      & \textbf{0.67}   & \textbf{0.78} &  397    \\ \hline\hline
%\multirow{5}{2cm}{Irish Water Charges}         & \multirow{5}{*}{8} & \multirow{5}{*}{10} & None & 8              & 10             & 0.78      & 0.64   & 0.71 & 45   \\ \cline{4-10} 
%                                             &                    &                     & Acc    & 700            & 2577           & 0.95      & 0.73   & 0.83 & 69   \\ \cline{4-10} 
%                                             &                    &                     & Rev    & 446            & 1818           & 0.97      & 0.73   & 0.83 & 1970 \\ \cline{4-10} 
%                                             &                    &                     & RR     & 653            & 2929           & 0.97      & 0.75   & 0.84 &   1645   \\ \cline{4-10} 
%                                             &                    &                     & AR     & 722            & 2676           & \textbf{0.97}      & \textbf{0.77}   & \textbf{0.86} &   282   \\ \hline\hline
%\multirow{5}{2cm}{Trump Healthcare}            & \multirow{5}{*}{5}  & \multirow{5}{*}{9}   & None &               5 &    9            & 0.60          & 0.60       &     0.60 & 43     \\ \cline{4-10} 
%                                             &                    &                     & Acc    & 58             & 94             & 0.66      & 0.65   & 0.64 &  24    \\ \cline{4-10} 
%                                             &                    &                     & Rev    & 93             & 177            & 0.65      & 0.64   & 0.63 &  863    \\ \cline{4-10} 
%                                             &                    &                     & RR     & 93             & 177            & 0.67      & 0.66   & 0.66 & 855     \\ \cline{4-10} 
%                                             &                    &                     & AR     & 75             & 145            & \textbf{0.69}      & \textbf{0.68}   & \textbf{0.67} &  99    \\ \hline\hline
%\multirow{5}{2cm}{London Attack}               & \multirow{5}{*}{3}  & \multirow{5}{*}{3}   & None &               3 &  3              & 0.80          &  0.60      &  0.69    &  12    \\ \cline{4-10} 
%                                             &                    &                     & Acc    & 190            & 402            & 0.81      & 0.62   & 0.70 &   15   \\ \cline{4-10} 
%                                             &                    &                     & Rev    & 234            & 617            & 0.80     & \textbf{0.70}   & \textbf{0.75} &   360   \\ \cline{4-10} 
%                                             &                    &                     & RR     & 170            & 351            & 0.81      & 0.68   & 0.73 &   360   \\ \cline{4-10} 
%                                             &                    &                     & AR     & 257            & 649            & \textbf{0.82}      & \textbf{0.70}   & \textbf{0.75} &  60    \\ \hline
%\end{longtable}
%\clearpage 
%}

\begin{table*}[]
\centering
\caption{Comparing the 5 semi-supervised selection (SSS) techniques using 8 test story datasets. The N and E refer to number of nodes and edges of the initial story graph $G_{t_0}$. The N$\prime$ and E$\prime$ refer to the number of nodes and edges of the updated story graph when reaching the end of stream $T$. Time refer to the running time of each method for the story and their corresponding test stream T, including both story updating time and document classification time.}
\label{table:sss-compare}
\begin{tabular}{|p{2cm}|c|c|c|c|c|c|c|c|c|}
\hline
Story                                        & N & E             & SSS    & N$\prime$ & E$\prime$ & Precision & Recall & F1   & Time(s) \\ \hline
\multirow{5}{2cm}{Cyclone Debbie}              & \multirow{5}{*}{9}  & \multirow{5}{*}{12}   & None & 9               & 12             & 0.91       & \textbf{1}     & 0.95    &    21  \\ \cline{4-10} 
                                             &                    &                     & Acc    & 99             & 313            & 0.93      & 0.98   & 0.96 &  8   \\ \cline{4-10} 
                                             &                    &                     & Rev    & 125            & 345            & 0.96       & 0.98   & 0.97 & 248  \\ \cline{4-10} 
                                             &                    &                     & RR     & 130            & 400            & \textbf{0.97}      & 0.98   & \textbf{0.98} &   234   \\ \cline{4-10} 
                                             &                    &                     & AR     & 97             & 307            & 0.95      & 0.98   & 0.96 &   30   \\ \hline\hline
\multirow{5}{2cm}{Kim Jong-Nam Death}          & \multirow{5}{*}{6}  & \multirow{5}{*}{9}   & None &               6 &    9            &  0.91         &   0.97     &     0.94 &   21   \\ \cline{4-10} 
                                             &                    &                     & Acc    & 96            & 433            & \textbf{0.97}      & 0.99    & \textbf{0.98}  &  21    \\ \cline{4-10} 
                                             &                    &                     & Rev    & 115            & 514            & \textbf{0.97}       & \textbf{1}    & \textbf{0.98}  &  777    \\ \cline{4-10} 
                                             &                    &                     & RR     & 98            & 393            & \textbf{0.97}       & \textbf{1}    & \textbf{0.98}  & 816     \\ \cline{4-10} 
                                             &                    &                     & AR     & 87             & 403            & \textbf{0.97}       & \textbf{1}    & \textbf{0.98}  &  102    \\ \hline\hline
\multirow{5}{2cm}{Orly Airport Attack}         & \multirow{5}{*}{4}  & \multirow{5}{*}{6}   & None &               4 &   6             &   0.92        &  0.95      &     0.93 &  12    \\ \cline{4-10} 
                                             &                    &                     & Acc    & 59             & 129             & 0.95     & \textbf{0.95}   & \textbf{0.95} &   10   \\ \cline{4-10} 
                                             &                    &                     & Rev    & 62             & 132            & \textbf{0.96}      & 0.91   & 0.93 &   404   \\ \cline{4-10} 
                                             &                    &                     & RR     & 67             & 165            & \textbf{0.96}      & 0.93   & \textbf{0.95} &   422   \\ \cline{4-10} 
                                             &                    &                     & AR     & 45             & 100             & 0.94      & 0.93   & 0.93 &   45   \\ \hline\hline
\multirow{5}{2cm}{South Africa President Zuma} & \multirow{5}{*}{8}  & \multirow{5}{*}{19}   & None &               8 & 19               &  0.80         &  0.84      &     0.80 &  5    \\ \cline{4-10} 
                                             &                    &                     & Acc    & 184            & 597            & 0.95      & 0.70   & 0.80 &  8    \\ \cline{4-10} 
                                             &                    &                     & Rev    & 167            & 642            & 0.95      & 0.57   & 0.72 &  89    \\ \cline{4-10} 
                                             &                    &                     & RR     & 126            & 440            & \textbf{0.96}      & 0.71   & 0.81 &   92   \\ \cline{4-10} 
                                             &                    &                     & AR     & 121            & 485            & \textbf{0.96}      & \textbf{0.71}   & \textbf{0.82} &   18   \\ \hline\hline
\multirow{5}{2cm}{EU Migrant Crisis}           & \multirow{5}{*}{2}  & \multirow{5}{*}{1}   & None &               2 &    1            &  \textbf{0.92}         &  0.47      &     0.62 & 61     \\ \cline{4-10} 
                                             &                    &                     & Acc    & 530            & 2091           & 0.91      & 0.57   & 0.70 &    68  \\ \cline{4-10} 
                                             &                    &                     & Rev    & 1024           & 4714           & 0.91      & \textbf{0.67}   & 0.77 &  2798    \\ \cline{4-10} 
                                             &                    &                     & RR     & 168            & 406            & 0.89      & 0.66   & 0.76 &  1534    \\ \cline{4-10} 
                                             &                    &                     & AR     & 873            & 4219           & \textbf{0.92}      & \textbf{0.67}   & \textbf{0.78} &  397    \\ \hline\hline
\multirow{5}{2cm}{Irish Water Charges}         & \multirow{5}{*}{8} & \multirow{5}{*}{10} & None & 8              & 10             & 0.78      & 0.64   & 0.71 & 45   \\ \cline{4-10} 
                                             &                    &                     & Acc    & 700            & 2577           & 0.95      & 0.73   & 0.83 & 69   \\ \cline{4-10} 
                                             &                    &                     & Rev    & 446            & 1818           & 0.97      & 0.73   & 0.83 & 1970 \\ \cline{4-10} 
                                             &                    &                     & RR     & 653            & 2929           & 0.97      & 0.75   & 0.84 &   1645   \\ \cline{4-10} 
                                             &                    &                     & AR     & 722            & 2676           & \textbf{0.97}      & \textbf{0.77}   & \textbf{0.86} &   282   \\ \hline\hline
\multirow{5}{2cm}{Trump Healthcare}            & \multirow{5}{*}{5}  & \multirow{5}{*}{9}   & None &               5 &    9            & 0.60          & 0.60       &     0.60 & 43     \\ \cline{4-10} 
                                             &                    &                     & Acc    & 58             & 94             & 0.66      & 0.65   & 0.64 &  24    \\ \cline{4-10} 
                                             &                    &                     & Rev    & 93             & 177            & 0.65      & 0.64   & 0.63 &  863    \\ \cline{4-10} 
                                             &                    &                     & RR     & 93             & 177            & 0.67      & 0.66   & 0.66 & 855     \\ \cline{4-10} 
                                             &                    &                     & AR     & 75             & 145            & \textbf{0.69}      & \textbf{0.68}   & \textbf{0.67} &  99    \\ \hline\hline
\multirow{5}{2cm}{London Attack}               & \multirow{5}{*}{3}  & \multirow{5}{*}{3}   & None &               3 &  3              & 0.80          &  0.60      &  0.69    &  12    \\ \cline{4-10} 
                                             &                    &                     & Acc    & 190            & 402            & 0.81      & 0.62   & 0.70 &   15   \\ \cline{4-10} 
                                             &                    &                     & Rev    & 234            & 617            & 0.80     & \textbf{0.70}   & \textbf{0.75} &   360   \\ \cline{4-10} 
                                             &                    &                     & RR     & 170            & 351            & 0.81      & 0.68   & 0.73 &   360   \\ \cline{4-10} 
                                             &                    &                     & AR     & 257            & 649            & \textbf{0.82}      & \textbf{0.70}   & \textbf{0.75} &  60    \\ \hline
\end{tabular}
\end{table*}

In this section, we evaluate the 4 semi-supervised selection (SSS) techniques. 
In Section \ref{sec:semi-supervised}, we describe 2 standard SSS approaches from semi-supervised learning: Accumulate (Acc) and Revisit (Rev), and we propose 2 new SSS methods: Revisit-Recent (RR) and Accumulate+Revisit (AR).
We compare these 4 methods to using no SSS solution, on the 8 test story datasets presented in Section \ref{sec:label-data}.

\textbf{Experiment Setup.} We simulate the story tracking process: given the \emph{seed docs} for a story, and a document stream $T$ (mix of articles and tweets), we classify the doc $m$, $m\in T$ into relevant or irrelevant to the story.
For each story of the 8 test stories, we first sort its labeled data by the publishing time, then we use the first relevant article of each story as the \emph{seed doc}, and the rest as the stream $T$.
The number of relevant articles and tweets per story are shown in Table \ref{table:9-stories-keyphrases-hashtags}. 
We have the same number of irrelevant articles and tweets in the stream as well.
We employ the L2R classifier trained with the 16.2K labeled data with all 13 features, and compare the performance of the 5 approaches using Precision, Recall, F1 and the total runtime.

\textbf{Result.} The experiment results are presented in Table \ref{table:sss-compare}. The 5 different SSS methods process each story. 
All methods use the same trained classifier, while the story representation (i.e., \emph{story docs} and entity graph $G$) are different between methods.
Because we only use a single article as the \emph{seed doc},
the first story entity graphs $G_{t_0}$ are very small (e.g., less than 10 nodes and less than 20 edges).
At the end of the stream $T$, depending on the stories and the SSS methods, the story entity graphs are extended to tens or hundreds of nodes and edges (i.e., N$\prime$ and E$\prime$).

The classification quality difference between the 5 SSS methods in the first 3 news stories is negligible.
We find these 3 stories are straightforward to track, because of their low story complexity.
These 3 stories have only one or two keyphrases that describe the story (e.g., cyclone debbie, kim jongnam), and almost all articles and tweets relevant to these story mentioned one of the keyphrases.
The classification quality of these 3 stories are good enough (e.g., F1 around 90\%) even using no SSS method.

Tracking the other 5 stories is more challenging. The EU Migrant Crisis, and the Irish Water Charges are two long running stories with articles and tweets gathered over a year.
During this period, the stories develop quite a lot with a rich amount of details reported on all aspects of the stories.
The Trump Healthcare story is one of the many sub-stories of Trump and US politics, and thus, is very hard to separate this particular healthcare story from other Trump stories.
The London Attack, on the other hand, is a short term, but a very popular story.
A huge amount of articles and tweets are posted on this topic, and thus, include many story details.

With no SSS method and using only one article as \emph{seed doc}, the L2R classifier already achieves around 0.70 in F1 when tracking these 5 complex stories.
Among the 4 SSS solutions, Acc takes less amount of time, but in general, is not as accurate as the other 3 approaches.
Rev and RR have good accuracy, but take an extremely long time, making them not suitable for our real-time requirement.
The proposed AR approach achieves the best accuracy-time trade-off.
It increases the F1 by 2.5\%, 25.8\%, 21.1\%, 11.6\%, 8.6\% for the 5 complex stories, a significant improvement compared to using no SSS solution.


\subsection{Comparing to Other Story Tracking Approaches}

In this experiment, we compare our model, Story Disambiguation, to state-of-the-art (SOTA) story tracking techniques.
There are two types of SOTA approaches: binary classification/topic modeling methods that consider documents from the target story as one class and irrelevant documents as another, and story clustering methods that cluster documents into small groups and consider each group as a story.
From our initial experiment results, we find the performance of clustering techniques is not as good as the classification approaches, because they are designed to detect the first story from the document stream, rather than tracking stories.
Hence, in this experiment, we only compare our model to binary classification approaches.
These methods require some amount of labeled documents per story, and use bag-of-words type features.
We simulate 3 variant binary classification approaches and compare to our Story Disambiguation framework:
\begin{enumerate}
    \item \textbf{Text  (T) \cite{allan1998topic,schultz1999topic,makkonen2004simple}:} A binary classifier is trained on the positive and negative labeled examples for the target story, using tf-idf bag-of-words feature vectors. We compare some classifiers and choose Logistic Regression (in scikit-learn lib) for its accuracy and fast runtime when given large feature vectors.
    \item \textbf{Entity (E):} Similar to the previous one, but instead of using text features, the classifier uses disambiguated entities as features. The feature vectors consist of the entity count of the labeled examples. In a short text streaming environment, such as Twitter data, this approach is only feasible with the support of the SOTA disambiguation techniques that are both accurate and work in real-time.
    \item \textbf{Text + Entity (T+E):} This method joins the Text and Entity approaches by directly combining the feature vectors of the two methods.
\end{enumerate}

We evaluate two versions of the Story Disambiguation framework:
\begin{enumerate}
    \item \textbf{Story Disambiguation (SD):} The standard Story Disambiguation framework without the semi-supervised selection (SSS) solution. SD uses an L2R ranking classifier trained on 16.2K labeled data gathered from ``Irish General Election 2016 (GE16)'' story. The training examples used by the SOTA approach are used as \emph{seed docs} in SD to represent the target story. The story entity graphs in this approach remain the same.
    \item \textbf{Story Disambiguation with Semi-Supervised Selection (SD+SSS):} The Story Disambiguation framework with SSS solution: Accumulate+Revisit (AR) as presented in Section \ref{sec:semi-supervised}. The story entity graphs in this approach are updated based on the predicted results of the L2R classifier.
\end{enumerate}

%As an evaluation metric, we use the standard Information Retrieval measurements: Precision, Recall, and F1. 

\subsubsection{Training Examples}


\begin{figure*}[]
    \centering 
    \includegraphics[width=1\linewidth]{story_figs/compare-sota-train-text.eps}
    \caption{Evaluating the F1 of the 5 methods given different number of positive training examples on the Irish Water Charges story. The type of training and testing data include: articles only, tweets only, and both articles and tweets. The last row uses a minimum of 1 article and 1 tweet as seed documents.}
    \label{fig:compare-sota-train-text}
\end{figure*}


We first study the impact of a different number of training examples, as well as mixed types of training and testing examples (e.g., mixing articles and tweets).

\textbf{Experiment Setup.} We first evaluate the 5 comparison methods on one story dataset, ``Irish Water Charges". 
The story dataset contains 750+ articles and 10K tweets with an equal number of relevant and irrelevant examples.
To analyze the behavior of the 5 methods on data from different domains, we set-up 9 test cases where the training and test data are the combinations of three types: articles only, tweets only, and both articles and tweets.
For instance, one test case is to train the 5 methods on tweets and test them on articles.

In each test case, we vary the number of positive training examples for training the methods from 1 to 12 examples.
For test cases that use both articles and tweets as training examples, we select the same amount of articles and tweets.
We first sort the story dataset by chronological order, then we select the first few examples as the training data, and the rest as the testing data (i.e., simulating the document stream $T$).
We measure the F1 of the 5 methods.

\textbf{Result.} The detailed experiment results of the 9 test cases are presented in Figure \ref{fig:compare-sota-train-text}. 
The first row of the plot matrix is for test cases trained on articles, while the second row is for tweets and the last row is for both articles and tweets.
Similarly, the first column is for test cases that are tested on articles, and the other two columns are for testing on tweets, and both articles and tweets.
Each plot shows the F1 value of the 5 methods trained on a different number of training examples.

In all 9 test cases, the Text approach needs around 10 positive training examples to reach a stable F1 of 0.80.
The Entity approach and Test+Entity approach behave similarly, requiring around 5 positive examples, showing the impact of disambiguation techniques in story tracking tasks.
Our proposed Story Disambiguation methods: SD and SD+SSS, provide good prediction results (0.80 - 0.85 in F1) with only 1 positive training example.
Thus, we out-perform the other approaches when very little labeled data are available.
This is due to the way we model the story tracking problem as an L2R problem.
By using a ranking classifier, we avoid retraining the model per target story, and thus, require less amount of labeled data to define the story.

We have some interesting findings regarding the types of training and testing data.
First of all, the SOTA approaches work well when trained and tested on the same types of data.
As shown in subplot (1,1) (i.e., the plot on the first row and first column) and (2,2) in Figure \ref{fig:compare-sota-train-text}, given enough training examples, the SOTA approaches out-perform the SD and SD+SSS when both trained and tested on articles or tweets.
On the other side, if training and testing data are different (e.g., plot (1,2) and (2,1)), the SOTA approaches are not performing as well.
The Text approach fails in such cases.
This is due to the bag-of-words type of features used in the Text approach, which is incapable of handling data of mixed language styles and vocabulary.
In comparison, Entity and Text+Entity approaches perform much better, because they use the entities in the documents, which are disambiguated in advanced, and are very effective in describing the target story at a higher level.

When trained and tested on mixed types of content (as shown in plot(3,3)), our proposed SD and SD+SSS approaches consistently out-perform the other 3 methods, with SD+SSS better than the SD.
Similarly to other test cases when the training and testing data is from different or mixed domains, SD and SD+SSS show stable prediction performance in F1 of 0.80 - 0.85, showing our model design is capable of tracking stories in multiple domains with different language style and vocabulary.

From the testing data perspective, regardless of the training data, articles are easier to track than tweets, with an average of 0.05 to 0.10 difference in F1 values.
Also, classifiers trained on articles are better in accuracy comparing to trained on tweets, due to the short and noisy nature of the tweets.


\subsubsection{Target Stories}

In this section, we evaluate the 5 methods on different types of stories.

\textbf{Experiment Setup.}
We use the 8 testing stories to compare the 5 methods, in two test cases.
Both cases use articles as training data, and both articles and tweets as testing data.
In one test case, there is only 1 positive example in the training set, while in the other test cases, there are 10.
Similar to the previous experiment, we sort the story datasets by chronological order, and use the first few documents as training data and the rest of documents as testing data.
We measure the Precision, Recall, and F1 of the 5 methods.
The amount of relevant articles and tweets for each story are presented in Table \ref{table:9-stories-keyphrases-hashtags}, and the attributes of the stories are presented in Table \ref{table:9-stories}.

\begin{table*}[]
\centering
\caption{Comparing the 5 methods on 8 story datasets in Precision, Recall, F1 and running time per document, with the classifiers trained on articles and tested on both articles and tweets.}
\label{table:compare-sota-stories}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c||c|c|c|c|c|}
\hline
\multirow{2}{2cm}{Story}                       & \multirow{2}{*}{} & \multicolumn{5}{c|}{Training: 1 Relevant Articles} & \multicolumn{5}{c||}{Training: 10 Relevant Articles}  \\ \cline{3-12} 
                                             &                   & T           & E             & T+E           & SD            & \footnotesize{SD+SSS}        & T             & E             & T+E           & SD            & \footnotesize{SD+SSS}        \\ \hline\hline
\multirow{3}{2cm}{Cyclone Debbie}              & P                 & \textbf{1}  & \textbf{1}    & \textbf{1}    & 0.91          & 0.95          & 0.99          & \textbf{1}    & \textbf{1}    & 0.95          & 0.95          \\ \cline{2-12} 
                                             & R                 & 0           & 0.96          & 0.96          & \textbf{1}    & 0.98          & 0.34          & 0.96          & 0.96          & \textbf{0.98} & \textbf{0.98} \\ \cline{2-12} 
                                             & F1                & 0           & \textbf{0.98} & \textbf{0.98} & 0.95          & 0.96          & 0.50          & \textbf{0.98} & \textbf{0.98} & 0.97          & 0.97          \\ \cline{2-12} 
                                             & Time(ms)          & 0.3           & 0.5          & 0.7          & 4.9          & 22.2                & 0.2      & 0.4          & 0.7          & 4.7          & 24.0          \\\hline
\multirow{3}{2cm}{Kim Jong-Nam Death}          & P                 & \textbf{1}  & \textbf{1}    & \textbf{1}    & 0.91          & 0.97          & 0.98          & \textbf{1}    & 0.99          & 0.93          & 0.98          \\ \cline{2-12} 
                                             & R                 & 0.01        & 0.90          & 0.90          & 0.97          & \textbf{1}    & 0.27          & 0.89          & 0.90          & 0.99          & \textbf{1}    \\ \cline{2-12} 
                                             & F1                & 0.02        & 0.94          & 0.94          & 0.94          & \textbf{0.98} & 0.42          & 0.94          & 0.95          & 0.96          & \textbf{0.99} \\ \cline{2-12} 
                                             & Time(ms)          & 0.2           & 0.3          & 0.7          & 4.7          & 41                & 0.2      & 0.4          & 0.7          & 4.5          & 42          \\\hline
\multirow{3}{2cm}{Orly Airport Attack}         & P                 & \textbf{1}  & \textbf{1}    & \textbf{1}    & 0.92          & 0.94          & \textbf{1}    & \textbf{1}    & \textbf{1}    & 0.92          & 0.95          \\ \cline{2-12} 
                                             & R                 & 0           & 0.64          & 0.64          & \textbf{0.95} & 0.93          & 0.49          & 0.63          & 0.64          & \textbf{0.91} & 0.89          \\ \cline{2-12} 
                                             & F1                & 0.01        & 0.78          & 0.78          & \textbf{0.93} & \textbf{0.93} & 0.66          & 0.77          & 0.78          & \textbf{0.92} & \textbf{0.92} \\ \cline{2-12} 
                                             & Time(ms)          & 0.1           & 0.5          & 0.6          & 3.8          & 25.9                & 0.2      & 0.4          & 0.6          & 4.7          & 32.5          \\\hline
\multirow{3}{2cm}{South Africa Zuma} & P                 & \textbf{1}  & 0.98          & 0.98          & 0.80          & 0.96          & \textbf{0.98} & 0.97          & 0.97          & 0.89          & 0.96          \\ \cline{2-12} 
                                             & R                 & 0.01        & 0.16          & 0.16          & \textbf{0.84} & 0.71          & 0.12          & 0.41          & 0.41          & \textbf{0.86} & 0.75          \\ \cline{2-12} 
                                             & F1                & 0.03        & 0.27          & 0.27          & 0.80          & \textbf{0.82} & 0.21          & 0.58          & 0.58          & \textbf{0.88} & 0.84          \\ \cline{2-12} 
                                             & Time(ms)          & 0.4           & 0.9          & 0.9          & 4.7          & 27                & 0.4      & 0.5          & 1.0          & 5.5          & 28.7          \\\hline
\multirow{3}{2cm}{EU Migrant Crisis}           & P                 & \textbf{1}  & 0.98          & 0.98          & 0.92          & 0.92          & \textbf{0.98} & 0.96          & 0.96          & 0.89          &  0.92           \\ \cline{2-12} 
                                             & R                 & 0           & 0.01          & 0.01          & 0.47          & 0.67          & 0.27          & 0.24          & 0.24          & 0.66        & \textbf{0.70}     \\ \cline{2-12} 
                                             & F1                & 0.01        & 0.02          & 0.02          & 0.62          & \textbf{0.78} & 0.42          & 0.38          & 0.39          & 0.76          & \textbf{0.80}   \\\cline{2-12} 
                                             & Time(ms)          & 0.6           & 1.3          & 1.4          & 4.7          & 110.7                & 0.6      & 0.5          & 1.2          & 5.1          & 120.8          \\ \hline
\multirow{3}{2cm}{Irish Water Charges}         & P                 & 0.75        & 0.83          & 0.91          & 0.78          & \textbf{0.97} & \textbf{0.99} & 0.51          & 0.91          & 0.80          & 0.89          \\ \cline{2-12} 
                                             & R                 & 0           & 0.04          & 0.03          & 0.64          & \textbf{0.77} & 0.31          & \textbf{0.99} & 0.85          & 0.77          & 0.79          \\ \cline{2-12} 
                                             & F1                & 0           & 0.07          & 0.06          & 0.71          & \textbf{0.86} & 0.47          & 0.67          & \textbf{0.88} & 0.78          & 0.84          \\ \cline{2-12} 
                                             & Time(ms)          & 0.1           & 0.1          & 0.2          & 1.1          & 67                & 0.3      & 0.4          & 0.9          & 4.3          & 74.8          \\\hline
\multirow{3}{2cm}{Trump Healthcare}            & P                 & \textbf{1}  & 0.53          & 0.53          & 0.60          & 0.69          & \textbf{0.90} & 0.56          & 0.56          & 0.70          & 0.70          \\ \cline{2-12} 
                                             & R                 & 0           & 0.10          & 0.10          & 0.60          & \textbf{0.68} & 0.05          & 0.12          & 0.12          & 0.59          & \textbf{0.68} \\ \cline{2-12} 
                                             & F1                & 0           & 0.16          & 0.16          & 0.60          & \textbf{0.67} & 0.10          & 0.20          & 0.20          & 0.64          & \textbf{0.68} \\ \cline{2-12} 
                                             & Time(ms)          & 0.2           & 0.6          & 0.7          & 4.6          & 42.5                & 0.2      & 0.4          & 0.7          & 4.8          & 43.3          \\\hline
\multirow{3}{2cm}{London Attack}               & P                 & \textbf{1}  & 0.92          & 0.92          & 0.80          & 0.82          & \textbf{0.94} & 0.50          & 0.80          & 0.82          & 0.82          \\ \cline{2-12} 
                                             & R                 & 0           & 0.07          & 0.07          & 0.60          & \textbf{0.70} & 0.49          & \textbf{0.97} & 0.78          & 0.62          & 0.63          \\ \cline{2-12} 
                                             & F1                & 0           & 0.12          & 0.12          & 0.69          & \textbf{0.75} & 0.65          & 0.66          & \textbf{0.79} & 0.71          & 0.72          \\ \cline{2-12} 
                                             & Time(ms)          & 0.3           & 0.8          & 0.9          & 4.7          & 33.7                & 0.3      & 0.4          & 0.8          & 4.7          & 34.4          \\\hline
\end{tabular}}
\end{table*}


\textbf{Result.} The Precision, Recall and F1 of the 5 methods on the 8 testing story dataset in the 2 test settings are shown in Table \ref{table:compare-sota-stories}.
%We also present the F1 values in Figure \ref{}.
%\todo{add a figure to present the results in table 5.8}
Comparing the 2 test settings, we see similar behaviors of the 5 methods as in the previous experiment: Text, Entity, and Text+Entity approaches do not work well when given only 1 positive training example.
Our proposed SD and SD+SSS on the other hand, have stable performance regardless of the number of positive training examples.

In terms of the 8 testing stories, we find that the stories of high complexity are harder to track.
For low complexity stories, Cyclone Debbie, Kim Jong-Nam Death and Orly Airport Attack, the Precision, Recall and F1 easily go beyond 0.95.
These stories are reported in the news with limited details and include fewer entities, and can be easily tracked with few story key phrases.
The relevant documents are similar to each other, thus making these stories simple tracking targets.

The other 5 stories are difficult to track, especially for the SOTA approaches. Given 1 positive training example, the SOTA approaches fail on these 5 stories. With 10 positive training examples, the F1 of these approaches are mostly below 0.70.
For instance, the F1 of Trump Healthcare story is below 0.20 for SOTA approaches, and F1 of EU Migrant Crisis is below 0.40.
This is partially due to the insufficient training data. 
For a complex story, training a classifier per target story requires more positive training examples to capture the story, and 10 of them are not enough.
Another reason is that these stories have a complex structure between story entities, and the bag-of-words types of features are incapable of capturing such relationship.

In comparison to SOTA approaches, SD and SD+SSS achieve much better F1. Given 10 positive training examples, their F1 is 0.30 higher than SOTA approaches in the South Africa President Zuma story, 0.40 higher in EU Migrant Crisis story, and 0.40 higher in the Trump Healthcare story.
Also, their tracking qualities are stable regardless of the number of positive training examples.
This is due to our modeling.
By using an L2R classifier, we avoid retraining the model for each target story, and require less positive training examples to define the story.
Also, we capture the story entity structure in a high-level entity graph, where the PageRank algorithm weights the entity importance.
Thus, our model can better handle the story details in the complex stories.
In average, SD+SSS has higher F1 compared to SD, showing the impact of the semi-supervised selection techniques.



